Is a Question Decomposition Unit All We Need?

Large Language Models (LMs) have achieved state-of-the-art performance on many Natural Language Processing (NLP) benchmarks. With the growing number of new benchmarks, we build bigger and more complex LMs. However, building new LMs may not be an ideal option owing to the cost, time and environmental impact associated with it. We explore an alternative route: can we modify data by expressing it in terms of the model's strengths, so that a question becomes easier for models to answer? We investigate if humans can decompose a hard question into a set of simpler questions that are relatively easier for models to solve. We analyze a range of datasets involving various forms of reasoning and find that it is indeed possible to significantly improve model performance (24% for GPT3 and 29% for RoBERTa-SQuAD along with a symbolic calculator) via decomposition. Our approach provides a viable option to involve people in NLP research in a meaningful way. Our findings indicate that Human-in-the-loop Question Decomposition (HQD) can potentially provide an alternate path to building large LMs. Code and data is available at https://github.com/Pruthvi98/QuestionDecomposition

==> tables/decomp_examples.tex <==
\begin{table*}[htp]
    \centering
    \begin{tabular}{c|p{30em}}
    \hline
    \multicolumn{2}{c}{Examples of decompositions for all the datasets}\\
    \hline
    
    \multirow{10}{*}{HotpotQA} & \textbf{\emph{Context}}: The Larkspur Press is a small letter-press publisher based in Monterey, Kentucky .... , The film also features appearances by Helen Keller, Anne Sullivan, Kate Adams Keller and Phillips Brooks Keller as themselves.  The movie was directed by George Foster Platt and written by Francis Trevelyan Miller.\\
    & \textbf{\emph{Original Question}}: Are John O'Hara and Rabindranath Tagore the same nationality?\\
    & \textbf{\emph{True Answer}}: no\\
    & \textbf{\emph{Decomposed Question 1}}: What is John O'Hara's nationality?\\
    & \textbf{\emph{Generated Answer}}: American\\
    & \textbf{\emph{Decomposed Question 2}}: What is Rbindranath Tagore's nationality?\\
    & \textbf{\emph{Generated Answer}}: Indian\\
    & \textbf{\emph{Decomposed Question 3}}: Is \#1 and \#2 the same nationality?\\
    & \textbf{\emph{Generated Answer}}: No\\
    \hline
    \multirow{9}{*}{SVAMP}& \textbf{\emph{Context}}: Bryan took a look at his books as well.If Bryan has 56.0 books in each of his 9.0 bookshelves.\\
    & \textbf{\emph{Original Question}}: How many books does he have in total?\\
    & \textbf{\emph{Answer}}: 504.0\\
    & \textbf{\emph{Decomposed Question 1}}:How many books in each bookshelf?\\
    & \textbf{\emph{Answer}}: 56.0\\
    & \textbf{\emph{Decomposed Question 2}}:How many bookshelves?\\
    & \textbf{\emph{Answer}}: 9.0\\
    & \textbf{\emph{Decomposed Question 3}}: multiplication ! \#1 ! \#2\\
    & \textbf{\emph{Answer}}: 504.0\\
    \hline
    \multirow{9}{*}{StrategyQA}& \textbf{\emph{Context}}: Mail carriers, also referred to as mailmen or letter carriers,  …  Clothing also provides protection from ultraviolet radiation.\\
    & \textbf{\emph{Original Question}}: True or False: Mail carriers need multiple uniforms.\\
    & \textbf{\emph{Original Answer}}: True\\
    & \textbf{\emph{Generated Answer}}: False\\
    & \textbf{\emph{Decomposed Question 1}}: What seasons do mail carriers work through?\\
    & \textbf{\emph{Generated Answer}}: All seasons\\
    & \textbf{\emph{Decomposed Question 2}}: True or False: In order to make it through all of \#1, one needs multiple clothing pieces.\\
    & \textbf{\emph{Generated Answer}}: True\\
    \hline
    \multirow{7}{*}{QASC}&\\
    & \textbf{\emph{Original Question}}: what kind of beads are formed from vapor condensing? (A) h2o (B) H20 (C) tiny (D) carbon (E) hydrogen (F) rain (G) oxygen (H) Dew\\
    & \textbf{\emph{Answer}}: h2o\\
    & \textbf{\emph{Decomposed Question 1}}: Are \#1 beads formed from vapor condensing?\\
    & \textbf{\emph{Answer}}: yes\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
